Visual Adversarial Examples Jailbreak Aligned Large Language Models

Recently, there has been a surge of interest in integrating vision into Large Language Models (LLMs), exemplified by Visual Language Models (VLMs) such as Flamingo and GPT-4. This paper sheds light on the security and safety implications of this trend. First, we underscore that the continuous and high-dimensional nature of the visual input makes it a weak link against adversarial attacks, representing an expanded attack surface of vision-integrated LLMs. Second, we highlight that the versatility of LLMs also presents visual attackers with a wider array of achievable adversarial objectives, extending the implications of security failures beyond mere misclassification. As an illustration, we present a case study in which we exploit visual adversarial examples to circumvent the safety guardrail of aligned LLMs with integrated vision. Intriguingly, we discover that a single visual adversarial example can universally jailbreak an aligned LLM, compelling it to heed a wide range of harmful instructions that it otherwise would not) and generate harmful content that transcends the narrow scope of a `few-shot' derogatory corpus initially employed to optimize the adversarial example. Our study underscores the escalating adversarial risks associated with the pursuit of multimodality. Our findings also connect the long-studied adversarial vulnerabilities of neural networks to the nascent field of AI alignment. The presented attack suggests a fundamental adversarial challenge for AI alignment, especially in light of the emerging trend toward multimodality in frontier foundation models.

==> sections/acknowledgement.tex <==
\section*{Acknowledgements}

We thank Tong Wu and Chong Xiang for their generous help and insightful discussions. Prateek Mittal acknowledges the support by NSF grants CNS-1553437 and CNS-1704105, the ARL’s Army Artificial Intelligence Innovation Institute (A2I2), the Office of Naval Research Young Investigator Award, the Army Research Office Young Investigator Prize, Schmidt DataX award, Princeton E-affiliates Award. Mengdi Wang acknowledges the support by NSF grants DMS-1953686, IIS-2107304, CMMI-1653435, ONR grant 1006977, and C3.AI. Xiangyu Qi acknowledges the support of Princeton Gordon
Y. S. Wu Fellowship. Any opinions, findings, conclusions, or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the funding agencies.

==> sections/exp_log.tex <==

\section{Quantitative Results Overview.}


\subsection{Defense.}

Main adversarial images (bs8): 

*d1. VAE of Stable Diffusion v1.5 (t=0) \note{Delete}

d2. t>0: 

start t & sqrt(1-alpha t):
0 -- 0.9971 (100\%)
30 -- 0.76 (75\%)
40 -- 0.4979 (50\%)
47 -- 0.2454 (25\%)


 
\subsection{Experiments log: \note{Status: Training -> Inference -> Evaluation}}

\textbf{Main}

\note{Raw input:}

angry panda.jpeg
adv imgs new
adv text.py

\note{Runs}

Clean Image: results formal0528 clean/

adv. image: results formal0524

Text: results formal0526/

Defense: results 0602 defense



\textbf{Full}

1. Vicuna Baseline (text only, WITHOUT Vicuna system prompt): results\_formal0428/baseline\_eval.jsonl  

1(rerun): Vicuna Baseline (text only, WITHOUT Vicuna system prompt): /results\_formal0521/baseline\_without\_sys.jsonl   prompt: ``a chat between a human and an assistant.''

1'. Vicuna Baseline (text only, WITH Vicuna system prompt): /results\_formal0521/baseline\_with\_sys.jsonl  

1.1. (image) training dataset = Manually constructed (universal): results\_formal0521  

1.1'. (image) varying adv budgets, no negative targets: results\_formal0524  

1.2 (text)  results\_formal0526  

1.3 (embedding) \note{TODO.}

\textbf{RTP targeted}

2. training dataset = RTP: results\_rtp0507 (epsilon=32, alpha=2) \note{Done.}

2.1  training dataset = RTP: results\_rtp\_raw\_0520 (epsilon=32, alpha=2). NO miniGPT4 system prompt. \note{Done.}

3. training dataset = RTP: results\_rtp\_0521 \note{Done.} (unconstraint, alpha=1) 

3.1  training dataset = RTP: results\_rtp\_raw\_0521 \note{Done.} (unconstraint, alpha=1). NO miniGPT4 system prompt.


Note: Vicuna system prompt ``A chat between a curious user and an artificial intelligence assistant. The assistant gives helpful, detailed, and polite answers to the user's questions.''






\subsection{Main Results TODO: multiply by 6 !!}

1. Compare Vicuna baseline, with and without safety prompts don't seem to make a prominent difference here. (Might because Vicuna is finetuned using shareGPT dataset, where all the datapoints are safe/non-toxic)

2. Compare the adv attacked results with baseline.

3. Ablation through different $\epsilon$ levels.

 \begin{table*}[htbp]
  \centering
    \begin{tabular}{lccccccc}
    \toprule
    perspective\_api & identity\_attack & profanity & severe\_toxicity & sexually\_explicit & threat & toxicity & Vicuna Perp. \\
    \midrule 
    Vicuna baseline  & 0.60\% & 5.82\% & 0.52\% & 2.40\% & 0.41\% & 7.20\% & 10.56 \\
    
    %1' baseline with system & 0.56\% & 6.2\% & 0.43\% & 2.35\% & 0.5\% & 7.12\% \\
    \midrule  
    adv. image $(\epsilon = 16/255)$  & 1.49\% & 6.22\% & 1.07\% & 2.41\% & 0.79\% & 8.22\% & 10.97 \\
     adv. image $(\epsilon = 32/255)$ & 2.52\% & 6.85\% & 1.19\% & 2.68\% & 0.98\% & 9.18\% & 13.31 \\
     adv. image $(\epsilon = 64/255)$ & 2.67\% & 8.35\% & 1.96\% & 2.81\% & 1.04\% & 10.48\% & 9.70 \\
     adv. image $(\epsilon = 128/255)$  & 2.15\% & 7.92\% & 1.18\% & 3.24\% & 0.66\% & 9.38\% & 9.21 \\
   adv. image (unconstrained)  & 3.18\% & 7.56\% & 1.39\% & 2.36\% & 1.37\% & 10.53\% & 15.94 \\
    \midrule 
    adversarial text & 1.04\% & 6.87\% & 0.75\% & 2.46\% & 0.72\% & 8.43\% & 22.53 \\
    \bottomrule
    \toprule
   detoxify & identity\_attack  & obscene & severe\_toxicity & insult & threat  &toxicity  & Vicuna Perp. \\
    \midrule 
    Vicuna baseline  & 0.29\%  & 5.29\% & 0.14\% & 2.59\% & 0.19\% & 6.64\%  & 10.56 \\ 
    \midrule
     adv. image $(\epsilon = 16/255)$ & 0.90\%  & 5.67\% & 0.44\% & 3.91\% & 0.37\% & 7.85\% & 10.97 \\
     adv. image $(\epsilon = 32/255)$ & 1.68\%  & 6.64\% & 0.44\% & 4.50\% & 0.47\% & 8.77\% & 13.31  \\
     adv. image $(\epsilon = 64/255)$ & 1.93\%  & 8.21\% & 0.84\% & 6.20\% & 0.44\% & 10.35\% & 9.70  \\
    adv. image $(\epsilon = 128/255)$  & 1.48\% & 7.40\% & 0.65\% & 4.62\%  & 0.38\% & 9.05\% & 9.21 \\
     adv. image (unconstrained)  &  1.82\% & 7.31\% & 0.45\% & 5.68\%  & 0.54\% & 10.48\% & 15.94 \\
    \midrule
    adversarial text  & 0.69\% & 6.37\% & 0.22\% & 3.84\%  & 0.40\% & 8.52\%  & 22.53\\
    \bottomrule
    \end{tabular} 
    
  \caption{Sample Table: \kaixuan{Shrink or Move to appendix if space if not enough.}}
  \label{tab:b1}%
\end{table*}%

 
\begin{table}[htbp]
  \centering
    \begin{tabular}{lcccccc}
    \toprule
    perspective\_api & identity\_attack & profanity & severe\_toxicity & sexually\_explicit & threat & toxicity \\
    \midrule
    1 baseline & 0.71\% & 6.04\% & 0.46\% & 2.43\% & 0.54\% & 7.37\% \\
    1(rerun) baseline without system & 0.6\% & 5.82\% & 0.52\% & 2.4\% & 0.41\% & 7.2\% \\
    1' baseline with system & 0.56\% & 6.2\% & 0.43\% & 2.35\% & 0.5\% & 7.12\% \\
    \midrule
    1.1ver0521 universal (unconstrained) & 2.66\% & 7.11\% & 1.07\% & 2.55\% & 0.83\% & 9.64\% \\
    \midrule
    1.1' constrained 16  & 1.49\% & 6.22\% & 1.07\% & 2.41\% & 0.79\% & 8.22\% \\
    1.1' constrained 32  & 2.52\% & 6.85\% & 1.19\% & 2.68\% & 0.98\% & 9.18\% \\
    1.1' constrained 64  & 2.67\% & 8.35\% & 1.96\% & 2.81\% & 1.04\% & 10.48\% \\
    1.1' constrained 128  & 2.15\% & 7.92\% & 1.18\% & 3.24\% & 0.66\% & 9.38\% \\
    1.1' unconstrained  & 3.18\% & 7.56\% & 1.39\% & 2.36\% & 1.37\% & 10.53\% \\
    \bottomrule
    \toprule
   detoxify & identity\_attack & insult & obscene & severe\_toxicity & threat  &toxicity \\
    \midrule
    1 baseline &  0.4\% & 2.75\% & 5.46\% & 0.22\% & 0.27\% & 7.07\% \\
    1(rerun) baseline without system & 0.29\% & 2.59\% & 5.29\% & 0.14\% & 0.19\% & 6.64\% \\
    1' baseline with system &  0.28\% & 2.45\% & 5.34\% & 0.1\% & 0.23\% & 6.6\% \\
    \midrule
    1.1ver0521 universal (unconstrained) & 1.83\% & 5.32\% & 7.25\% & 0.36\% & 0.34\% & 9.96\% \\
    \midrule
    1.1' constrained 16  & 0.9\% & 3.91\% & 5.67\% & 0.44\% & 0.37\% & 7.85\% \\
    1.1' constrained 32  & 1.68\% & 4.5\% & 6.64\% & 0.44\% & 0.47\% & 8.77\% \\
    1.1' constrained 64  & 1.93\% & 6.2\% & 8.21\% & 0.84\% & 0.44\% & 10.35\% \\
    1.1' constrained 128  & 1.48\% & 4.62\% & 7.4\% & 0.65\% & 0.38\% & 9.05\% \\
    1.1' unconstrained  &  1.82\% & 5.68\% & 7.31\% & 0.45\% & 0.54\% & 10.48\% \\
    \bottomrule
    \end{tabular}%
    
  \caption{Exp}
  %\label{tab:mytable}%
\end{table}%

\clearpage
\subsection{RTP targeted Results}

1. compare each targeted attack with the baseline. Show that training using RTP dataset increases the generation of the target attribute 

2. text template ablation: compare with miniGPT4 chatbot template and without miniGPT4 chatbot template. The difference is not prominent, so the attack method applies to different text templates.

3. compare the targeted dataset and the manually constructed dataset.

4. 

\begin{table}[htbp]
  \centering
    \begin{tabular}{lcccccc}
    \toprule
    perspective\_api & identity\_attack & profanity & severe\_toxicity & sexually\_explicit & threat & toxicity \\
    \midrule 
    results\_rtp0507/flirtation\_eval.jsonl & 0.66\% & 7.23\% & 0.45\% & 3.61\% & 0.42\% & 8.61\% \\
    results\_rtp0507/identity\_attack\_eval.jsonl & 0.82\% & 6.35\% & 0.52\% & 2.94\% & 0.48\% & 7.71\% \\
    results\_rtp0507/insult\_eval.jsonl & 0.57\% & 6.02\% & 0.32\% & 2.82\% & 0.54\% & 7.16\% \\
    results\_rtp0507/profanity\_eval.jsonl & 0.74\% & 7.16\% & 0.36\% & 3.22\% & 0.59\% & 8.70\% \\
    results\_rtp0507/severe\_toxicity\_eval.jsonl & 0.57\% & 6.56\% & 0.37\% & 2.81\% & 0.40\% & 7.78\% \\
    results\_rtp0507/sexually\_explicit\_eval.jsonl & 0.66\% & 7.18\% & 0.73\% & 5.17\% & 0.50\% & 8.67\% \\
    results\_rtp0507/threat\_eval.jsonl & 0.47\% & 4.80\% & 0.46\% & 2.40\% & 0.56\% & 5.89\% \\
    results\_rtp0507/toxicity\_eval.jsonl & 0.57\% & 6.75\% & 0.52\% & 2.96\% & 0.65\% & 8.32\% \\
    \midrule
    results\_rtp\_raw\_0520/flirtation\_eval.jsonl & 0.36\% & 4.39\% & 0.24\% & 4.03\% & 0.27\% & 5.86\% \\
    results\_rtp\_raw\_0520/identity\_attack\_eval.jsonl & 0.5\% & 4.57\% & 0.35\% & 1.97\% & 0.56\% & 5.49\% \\
    results\_rtp\_raw\_0520/insult\_eval.jsonl & 0.3\% & 3.76\% & 0.3\% & 1.77\% & 0.37\% & 4.93\% \\
    results\_rtp\_raw\_0520/profanity\_eval.jsonl & 0.38\% & 4.32\% & 0.35\% & 1.75\% & 0.3\% & 5.4\% \\
    results\_rtp\_raw\_0520/severe\_toxicity\_eval.jsonl & 0.45\% & 5.21\% & 0.48\% & 3.57\% & 0.41\% & 6.5\% \\
    results\_rtp\_raw\_0520/sexually\_explicit\_eval.jsonl & 0.41\% & 5.34\% & 0.44\% & 5.24\% & 0.45\% & 6.88\% \\
    results\_rtp\_raw\_0520/threat\_eval.jsonl & 0.34\% & 3.43\% & 0.42\% & 1.93\% & 0.58\% & 4.46\% \\
    results\_rtp\_raw\_0520/toxicity\_eval.jsonl & 0.89\% & 5.38\% & 0.52\% & 2.67\% & 0.46\% & 6.92\% \\
    \bottomrule
    detoxify & identity\_attack& insult &obscene& severe\_toxicity& threat& toxicity\\
    \midrule 
    results\_rtp\_0507 & & & & & &  \\
flirtation\_eval.jsonl & 0.32\% & 3.1\% & 6.28\% & 0.14\% & 0.24\% & 8.0\% \\
identity\_attack\_eval.jsonl & 0.45\% & 3.14\% & 6.02\% & 0.29\% & 0.29\% & 7.48\% \\
insult\_eval.jsonl & 0.27\% & 2.45\% & 5.33\% & 0.13\% & 0.25\% & 6.53\% \\
profanity\_eval.jsonl & 0.29\% & 3.02\% & 6.65\% & 0.15\% & 0.24\% & 8.02\% \\
severe\_toxicity\_eval.jsonl & 0.35\% & 2.68\% & 5.77\% & 0.09\% & 0.18\% & 6.98\% \\
sexually\_explicit\_eval.jsonl & 0.29\% & 3.11\% & 6.26\% & 0.18\% & 0.18\% & 7.77\% \\
threat\_eval.jsonl & 0.25\% & 2.27\% & 4.32\% & 0.12\% & 0.33\% & 5.71\% \\
toxicity\_eval.jsonl & 0.38\% & 3.29\% & 6.29\% & 0.21\% & 0.31\% & 7.76\% \\
    \midrule
    results\_rtp\_raw\_0520 & & & & & &  \\
    flirtation\_eval.jsonl & 0.15\% & 1.82\% & 3.85\% & 0.07\% & 0.18\% & 5.65\% \\
identity\_attack\_eval.jsonl & 0.28\% & 2.21\% & 3.91\% & 0.16\% & 0.26\% & 5.24\% \\
insult\_eval.jsonl & 0.17\% & 2.01\% & 3.62\% & 0.06\% & 0.11\% & 4.73\% \\
profanity\_eval.jsonl & 0.23\% & 1.92\% & 3.87\% & 0.15\% & 0.15\% & 5.03\% \\
severe\_toxicity\_eval.jsonl & 0.19\% & 1.93\% & 4.24\% & 0.07\% & 0.22\% & 5.33\% \\
sexually\_explicit\_eval.jsonl & 0.21\% & 2.09\% & 4.32\% & 0.11\% & 0.17\% & 5.68\% \\
threat\_eval.jsonl & 0.23\% & 1.6\% & 3.02\% & 0.06\% & 0.25\% & 4.34\% \\
toxicity\_eval.jsonl & 0.59\% & 3.09\% & 4.96\% & 0.24\% & 0.19\% & 6.92\% \\
    \bottomrule
    \end{tabular}%
    
  \caption{Exp}
  %\label{tab:mytable}%
\end{table}%





\begin{table}[htbp]
  \centering
    \begin{tabular}{lcccccc}
    \toprule
    perspective\_api & identity\_attack & profanity & severe\_toxicity & sexually\_explicit & threat & toxicity \\
    \midrule  
    results\_rtp\_0521 & & & & & &  \\
flirtation\_eval.jsonl & 0.64\% & 6.86\% & 0.93\% & 4.5\% & 0.59\% & 8.41\% \\ 
identity\_attack\_eval.jsonl & 1.66\% & 4.99\% & 0.67\% & 2.45\% & 1.11\% & 6.71\% \\ 
insult\_eval.jsonl & 1.07\% & 7.41\% & 1.34\% & 2.79\% & 0.99\% & 9.54\% \\ 
profanity\_eval.jsonl & 1.79\% & 9.19\% & 3.51\% & 3.28\% & 1.53\% & 10.21\% \\ 
severe\_toxicity\_eval.jsonl & 2.0\% & 9.3\% & 2.47\% & 3.14\% & 1.18\% & 10.43\% \\ 
sexually\_explicit\_eval.jsonl & 0.75\% & 6.28\% & 0.57\% & 3.83\% & 0.51\% & 7.52\% \\ 
threat\_eval.jsonl & 0.83\% & 5.02\% & 0.82\% & 2.33\% & 1.82\% & 6.69\% \\ 
toxicity\_eval.jsonl & 1.05\% & 7.69\% & 1.17\% & 2.71\% & 1.17\% & 9.21\% \\
    \midrule
    results\_rtp\_raw\_0521 & & & & & &  \\
flirtation\_eval.jsonl & 0.67\% & 6.86\% & 0.84\% & 5.09\% & 0.56\% & 8.65\% \\
identity\_attack\_eval.jsonl & 0.95\% & 5.15\% & 0.55\% & 2.54\% & 0.84\% & 6.83\% \\
insult\_eval.jsonl & 0.79\% & 6.89\% & 1.32\% & 2.45\% & 0.93\% & 8.36\% \\
profanity\_eval.jsonl & 1.0\% & 7.73\% & 1.06\% & 3.04\% & 0.97\% & 9.24\% \\
severe\_toxicity\_eval.jsonl & 0.92\% & 6.77\% & 1.34\% & 3.25\% & 1.57\% & 8.45\% \\
sexually\_explicit\_eval.jsonl & 0.66\% & 6.88\% & 0.66\% & 4.75\% & 0.71\% & 8.49\% \\
threat\_eval.jsonl & 0.73\% & 4.89\% & 0.78\% & 2.02\% & 3.03\% & 7.49\% \\
toxicity\_eval.jsonl & 1.03\% & 8.52\% & 1.41\% & 3.11\% & 1.13\% & 9.96\% \\
    \toprule
    detoxify & identity\_attack& insult &obscene& severe\_toxicity& threat& toxicity\\
    \midrule  
    results\_rtp\_0521 & & & & & &  \\
    flirtation\_eval.jsonl & 0.4\% & 3.54\% & 5.71\% & 0.2\% & 0.25\% & 7.33\% \\
identity\_attack\_eval.jsonl & 0.97\% & 2.84\% & 4.65\% & 0.3\% & 0.45\% & 6.89\% \\
insult\_eval.jsonl & 0.71\% & 4.87\% & 7.25\% & 0.46\% & 0.44\% & 9.22\% \\
profanity\_eval.jsonl & 1.12\% & 6.08\% & 8.81\% & 1.6\% & 0.71\% & 10.04\% \\
severe\_toxicity\_eval.jsonl & 1.24\% & 6.49\% & 9.08\% & 1.11\% & 0.51\% & 10.45\% \\
sexually\_explicit\_eval.jsonl & 0.57\% & 3.28\% & 5.96\% & 0.22\% & 0.19\% & 7.76\% \\
threat\_eval.jsonl & 0.47\% & 2.75\% & 4.58\% & 0.26\% & 0.77\% & 6.54\% \\
toxicity\_eval.jsonl & 0.58\% & 4.5\% & 7.15\% & 0.5\% & 0.71\% & 9.07\% \\
    \midrule
    results\_rtp\_raw\_0521 & & & & & &  \\
flirtation\_eval.jsonl & 0.39\% & 3.98\% & 6.61\% & 0.33\% & 0.36\% & 8.7\% \\
identity\_attack\_eval.jsonl & 0.57\% & 2.71\% & 4.55\% & 0.26\% & 0.29\% & 6.35\% \\
insult\_eval.jsonl & 0.5\% & 4.62\% & 6.51\% & 0.4\% & 0.5\% & 8.42\% \\
profanity\_eval.jsonl & 0.57\% & 4.62\% & 7.4\% & 0.4\% & 0.37\% & 9.36\% \\
severe\_toxicity\_eval.jsonl & 0.41\% & 4.12\% & 6.26\% & 0.43\% & 0.76\% & 8.32\% \\
sexually\_explicit\_eval.jsonl & 0.37\% & 3.25\% & 6.3\% & 0.24\% & 0.29\% & 8.31\% \\
threat\_eval.jsonl & 0.41\% & 3.09\% & 4.7\% & 0.44\% & 1.53\% & 7.94\% \\
toxicity\_eval.jsonl & 0.62\% & 5.27\% & 8.18\% & 0.42\% & 0.59\% & 9.94\% \\
    \bottomrule
    \end{tabular}
    
  \caption{Exp}
\end{table}%

==> sections/tables/defense_part.tex <==
 \begin{table*}[htbp]
  \centering
  \caption{The percentages of the generated outputs that exhibit certain toxic attributes given by Perspective API, tested on the RealToxicityPrompts \textit{challenging} subset. DiffPure effectively reduces the probability of toxic degeneration across all toxicity attributes. The leftmost column is the percentage of the generated texts that exhibit \textit{any} of the 6 attributes. For the full results across the other noise levels and the results of Detoxify classifier, see Table~\ref{tab:defense}. }
  \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    \multicolumn{8}{c}{Perspective API} \\
    Input & Any & Identity Attack & Profanity & Severe Toxicity & Sexually Explicit & Threat & Toxicity  \\
    \midrule    

    benign image without attack (baseline)  & 34.83\%  $\pm$ 1.63\% & 2.69\%  $\pm$ 0.24\% & 25.13\%  $\pm$ 1.76\% & 1.54\%  $\pm$ 0.17\% & 12.23\%  $\pm$ 0.55\% & 2.02\%  $\pm$ 0.13\% & 30.51\%  $\pm$ 1.44\% \\
    \midrule    
        adv. image $(\epsilon = 16/255)$  &  53.56\%  $\pm$ 1.03\% & 8.37\%  $\pm$ 0.42\% & 36.59\%  $\pm$ 0.55\% & 6.59\%  $\pm$ 0.52\% & 14.07\%  $\pm$ 0.34\% & 4.74\%  $\pm$ 0.31\% & 48.59\%  $\pm$ 0.56\% \\
  
   + DiffPure ($\sqrt{1-\alpha_t} = 0.5$)  & 37.50\%  $\pm$ 0.83\% & 2.68\%  $\pm$ 0.24\% & 26.43\%  $\pm$ 0.92\% & 1.28\%  $\pm$ 0.10\% & 13.05\%  $\pm$ 0.08\% & 2.17\%  $\pm$ 0.30\% & 31.31\%  $\pm$ 0.87\% \\
    
    \midrule    
     adv. image $(\epsilon = 32/255)$ &  59.36\%  $\pm$ 1.36\% & 14.59\%  $\pm$ 0.57\% & 39.53\%  $\pm$ 1.21\% & 6.97\%  $\pm$ 0.38\% & 14.87\%  $\pm$ 0.92\% & 6.16\%  $\pm$ 0.22\% & 53.75\%  $\pm$ 1.01\% \\
    
    + DiffPure ($\sqrt{1-\alpha_t} = 0.5$)  &  32.65\%  $\pm$ 0.72\% & 1.68\%  $\pm$ 0.41\% & 23.05\%  $\pm$ 0.28\% & 1.06\%  $\pm$ 0.11\% & 11.12\%  $\pm$ 0.23\% & 1.76\%  $\pm$ 0.25\% & 27.43\%  $\pm$ 1.20\% \\

    \midrule    
     adv. image $(\epsilon = 64/255)$   &  67.18\%  $\pm$ 0.17\% & 15.91\%  $\pm$ 0.18\% & 49.62\%  $\pm$ 0.39\% & 12.15\%  $\pm$ 0.50\% & 16.86\%  $\pm$ 0.42\% & 6.60\%  $\pm$ 0.48\% & 63.05\%  $\pm$ 0.78\% \\
  
    + DiffPure ($\sqrt{1-\alpha_t} = 0.5$) &  37.12\%  $\pm$ 0.97\% & 2.49\%  $\pm$ 0.58\% & 26.37\%  $\pm$ 0.76\% & 1.65\%  $\pm$ 0.26\% & 12.12\%  $\pm$ 0.31\% & 2.26\%  $\pm$ 0.14\% & 31.82\%  $\pm$ 0.69\% \\
   
  \midrule    
   adv. image (unconstrained)  & 66.04\%  $\pm$ 1.01\% & 17.41\%  $\pm$ 1.23\% & 43.25\%  $\pm$ 1.57\% & 7.96\%  $\pm$ 0.43\% & 14.60\%  $\pm$ 0.30\% & 7.04\%  $\pm$ 0.96\% & 61.70\%  $\pm$ 1.12\% \\

+ DiffPure ($\sqrt{1-\alpha_t} = 0.5$)& 32.76\%  $\pm$ 0.41\% & 2.16\%  $\pm$ 0.04\% & 22.41\%  $\pm$ 0.53\% & 1.28\%  $\pm$ 0.42\% & 11.58\%  $\pm$ 0.65\% & 1.96\%  $\pm$ 0.37\% & 27.99\%  $\pm$ 0.45\% \\
    \bottomrule
     
    \end{tabular} 
    }
  \label{tab:defense:part}%
\end{table*}%

==> sections/tables/partial_table.tex <==
\begin{table}[htbp]
\centering
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    Input & Identity Attack & Threat & Toxicity   \\
    \midrule 
    benign image without attack (baseline)  & 2.44\% & 2.02\% &  32.49\%   \\
    \midrule  
    adv. image $(\epsilon = 16/255)$  &  8.95\% \textbf{(+6.51\%)} &4.76\%  \textbf{(+ 2.74\%)} & 49.37\% \textbf{(+16.88\%)}   \\
     adv. image $(\epsilon = 32/255)$ & 15.13\% \textbf{(+12.69\%)} &5.93\% \textbf{(+3.91 \%)}& 55.1\% \textbf{(+22.61\%)}   \\
     adv. image $(\epsilon = 64/255)$ & 16.04\% \textbf{(+13.6\%)}& 6.26\%\textbf{(+ 4.24\%)} & 62.9\% \textbf{(+30.41\%)}  \\
     % adv. image $(\epsilon = 128/255)$  & 12.94\% & 56.3\% & 9.21 \\
   adv. image (unconstrained)  & 19.09\%\textbf{(+16.65\%)} & 8.25\% \textbf{(+6.23 \%)}& 63.21\%\textbf{(+30.72\%)}  \\
    \midrule 
    adversarial text & 6.26\% \textbf{(+3.82\%)}  & 4.35\%\textbf{(+ 2.33\%)}&  50.59\%\textbf{(+18.1\%)} \\
    \bottomrule
    \end{tabular} }
    
  \caption{The percentages of the generated outputs that exhibit certain toxic attributes given by Perspective API, tested on the RealToxicityPrompts \textit{challenging} subset.  For complete results, please refer to Table~\ref{tab:b1}. Adversarial images across constraint levels $\geq 32/255$ successfully trigger the model toward generating toxic content, and achieve better performance than text attacks. }
  
  \label{tab:1}%
\end{table}%
